Independent Languages and Witnesses of Dependence (Non-satisfaction)

We consider the independent language property defined by the language equation Ï†(X)=\emptyset, where the expression Ï† involves the language variable X, constant languages, and standard regular operations including transductions, but not complementation. This property consists of all languages L satisfying Ï†(L)=\emptyset. Depending on the choice of the operations in Ï†, the equation defines a broad class of codes, including combinations of standard variable-length codes and error-detecting codes. We show that any Ï†-independence is a JÃ¼rgensen independence, we define what a witness of non-satisfaction of Ï†(X)=\emptyset is, for a language L, and we show how to compute a witness of non-satisfaction when L is regular. We also discuss the complexity of the problem, showing that the decision version of the problem is PSPACE-complete.

==> eptcsdata.tex <==
\providecommand{\firstpage}{201}
\providecommand{\publicationstatus}{M. Hospod\'ar et al. (Eds.): 17th International Conference \\on Automata and Formal Languages (AFL 2026)\\
EPTCS 451, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.451.14}{10.4204/EPTCS.451.14}}
\pdfoutput=1

